DexBERT: Effective, Task-Agnostic and Fine-grained Representation Learning of Android Bytecode

The automation of a large number of software engineering tasks is becoming possible thanks to Machine Learning (ML). Central to applying ML to software artifacts (like source or executable code) is converting them into forms suitable for learning. Traditionally, researchers have relied on manually selected features, based on expert knowledge which is sometimes imprecise and generally incomplete. Representation learning has allowed ML to automatically choose suitable representations and relevant features. Yet, for Android-related tasks, existing models like apk2vec focus on whole-app levels, or target specific tasks like smali2vec, which limits their applicability. Our work is part of a new line of research that investigates effective, task-agnostic, and fine-grained universal representations of bytecode to mitigate both of these two limitations. Such representations aim to capture information relevant to various low-level downstream tasks (e.g., at the class-level). We are inspired by the field of Natural Language Processing, where the problem of universal representation was addressed by building Universal Language Models, such as BERT, whose goal is to capture abstract semantic information about sentences, in a way that is reusable for a variety of tasks. We propose DexBERT, a BERT-like Language Model dedicated to representing chunks of DEX bytecode, the main binary format used in Android applications. We empirically assess whether DexBERT is able to model the DEX language and evaluate the suitability of our model in three distinct class-level software engineering tasks: Malicious Code Localization, Defect Prediction, and Component Type Classification. We also experiment with strategies to deal with the problem of catering to apps having vastly different sizes, and we demonstrate one example of using our technique to investigate what information is relevant to a given task.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> biography.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/photo_tiezhu.png}}]
{Tiezhu Sun}
received his master's degree from Shandong University, and was mainly engaged in the research of deep learning and computer vision. He is currently a PhD student at the University of Luxembourg. His work mainly involves Software Engineering and Artificial Intelligence, especially Android Representation and Deep Learning Algorithms. His works were published at major conferences such as International Joint Conferences on Artificial Intelligence, AAAI Conference on Artificial Intelligence, International Conference on Pattern Recognition. \end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/kevin.png}}]{Kevin Allix}
Kevin Allix is an Associate Professor at CentraleSupélec, France.
He conducts research on Android Malware detection, Machine-Learning for Security, Software Engineering, and Natural Language Processing.
Kevin received his PhD degree in 2015 from the University of Luxembourg, and has been a post-doc for over five years at the SnT interdisciplinary centre of the University of Luxembourg. 
Kevin also held operational positions in network, system, and security engineering, and was an IT Security and Risk analyst for a private bank.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,clip]{figures/photo_kisub.jpeg}}]
{Kisub Kim}
received a Ph.D. degree in computer science from the University of Luxembourg in 2021. He is a research scientist at Singapore Management University. His work is mainly related to Software Engineering, broadly source code analysis and, specifically, code search, bug localization, code review, and code representation. 
His works were presented at major conferences such as International Conference on Software Engineering and published in top journals such as Empirical Software Engineering.
He has served as a reviewer, program committee, and organization committee in various software engineering conferences and journals, such as IEEE Transactions on Software Engineering, Empirical Software Engineering, and IEEE/ACM International Conference on Program Comprehension. 
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/photo_xin.JPG}}]
{Xin Zhou}
is a Ph.D. student at Singapore Management University, Singapore. His research interest is in code representation and software activity automation such as maintenance, debugging, or code reviewing. He is currently focusing on designing novel pre-trained code representations and applying them to automate developer-intensive activities.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/photo_dongsun.jpeg}}]
{Dongsun Kim}
is an assistant professor at Kyungpook National University. He has received his Ph.D. degree in Computer Science and Engineering from Sogang University, Korea. His career includes several academic and industrial experiences.
% He was a postdoctoral fellow at the Hong Kong University of Science and Technology from September 2010 to June 2013. He joined the University of Luxembourg as a research associate in November 2013 and continued his position until November 2018. From April 2019, he worked as a senior software test engineer position at Furiosa.ai. %, a fabless startup company manufacturing neural processing units.
He has published several research papers and participated in several research projects relevant to AI-based software engineering. 
% In particular, he has pioneered a new line of research on pattern-based program repair.
His recent achievements have focused on automated fix pattern mining, deep code representation for mining fix patterns, program repair driven by bug reports, fault localization impact on program repair, and specific topics for program repair.
% ; for these topics, he leveraged several AI-based techniques such as autoencoders, CNNs, etc.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,clip]{figures/photo_david.jpg}}]
{David Lo} is a Professor of Computer Science and Director of the Information and Systems Cluster at School of Computing and Information Systems, Singapore Management University. He leads the Software Analytics Research (SOAR) group. His research interest is in the intersection of software engineering, cybersecurity, and data science, encompassing socio-technical aspects and analysis of different kinds of software artifacts, with the goal of improving software quality and security and developer productivity.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bissyande.jpg}}]
{Tegawendé F. Bissyandé} 
is an associate professor with SnT, University of Luxembourg where he leads a group of 25 researchers. 
He is an ERC Fellow and Principal Investigator of several projects funded by the European Commission, the Fonds National de la Recherche, and by Industry partners.
His main interests are in Software Repair and Software Security with techniques based on program analysis and machine learning.
He has published over 80 peer-reviewed research papers in various fields of computer science.
As a native of Burkina Faso (West Africa), he is an enthusiastic advocate of capacity building for Higher education in Africa.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/photo-jacques.jpeg}}]
{Jacques Klein}
is an associate professor with SnT, University of Luxembourg. He co-leads a group of about 25 researchers focusing on Software Security, Software Reliability, and Intelligent Software. He has standing experience and expertise in (1) successfully running industrial projects, (2) Android security, including both static analysis techniques for tracking privacy leaks and machine learning for identifying malware, and (3) program repair. He published over 150 research papers in top journals/conferences.
\end{IEEEbiography}

